A Novel Pilot Allocation Technique for Uplink OFDMA in ISAC Systems

In integrated sensing and communication (ISAC) systems, pilot signals play a crucial role in enhancing sensing performance due to their strong autocorrelation properties and high transmission power. However, conventional interleaved pilots inherently constrain the maximum unambiguous range and reduce the accuracy of channel impulse response (CIR) estimation compared to continuous orthogonal frequency-division multiple access (OFDMA) signals. To address this challenge, we propose a novel overlapped block-pilot structure for uplink OFDMA-based ISAC systems, called phase-shifted ISAC (PS-ISAC) pilot allocation. The proposed method leverages a cyclic prefix (CP)-based phase-shifted pilot design, enabling efficient multi-transmitter pilot separation at the receiver. Simulation results confirm that the proposed scheme enhances CIR separation, reduces computational complexity, and improves mean square error (MSE) performance under practical power constraints. Furthermore, we demonstrate that utilizing continuous pilot resources maximizes the unambiguous range.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{UE}[UE]{user equipment}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{ISAC}[ISAC]{integrated sensing and communications}
\acrodef{IFFT}[IFFT]{inverse FFT}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{LS}[LS]{least-square}
\acrodef{MMSE}[MMSE]{minimum mean-square error}
\acrodef{BPSK}[BPSK]{binary phase shift keying}
\acrodef{CI-ISAC}[CI-ISAC]{conventional interleaved-ISAC}
\acrodef{PS-ISAC}[PS-ISAC]{phase-shifted-ISAC}
\acrodef{MSE}[MSE]{mean-square error}
\acrodef{NOMA}[NOMA]{non-orthogonal multiple access}
\acrodef{OOBE}[OOBE]{out-of-band emissions}
\acrodef{OFDMA}[OFDMA]{orthogonal frequency-division multiple access}
\acrodef{CFR}[CFR]{channel frequency response}
\acrodef{FPR}[FPR]{full pilot ratio}
\acrodef{PR}[PR]{pilot ratio}
\acrodef{MUR}[MUR]{maximum unambiguous range}
\acrodef{MA}[MA]{multiple access}
\acrodef{NGMA}[NGMA]{next-generation MA}
\acrodef{PRS}[PRS]{positioning reference signals}
\acrodef{UL}[UL]{uplink}
\acrodef{DL}[DL]{downlink}
\acrodef{CC}[CC]{computational complexity}
\acrodef{PC}[PC]{power constraints}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
